Multi-Camera Hand-Eye Calibration for Human-Robot Collaboration in Industrial Robotic Workcells

In industrial scenarios, effective human-robot collaboration relies on multi-camera systems to robustly monitor human operators despite the occlusions that typically show up in a robotic workcell. In this scenario, precise localization of the person in the robot coordinate system is essential, making the hand-eye calibration of the camera network critical. This process presents significant challenges when high calibration accuracy should be achieved in short time to minimize production downtime, and when dealing with extensive camera networks used for monitoring wide areas, such as industrial robotic workcells. Our paper introduces an innovative and robust multi-camera hand-eye calibration method, designed to optimize each camera's pose relative to both the robot's base and to each other camera. This optimization integrates two types of key constraints: i) a single board-to-end-effector transformation, and ii) the relative camera-to-camera transformations. We demonstrate the superior performance of our method through comprehensive experiments employing the METRIC dataset and real-world data collected on industrial scenarios, showing notable advancements over state-of-the-art techniques even using less than 10 images. Additionally, we release an open-source version of our multi-camera hand-eye calibration algorithm at https://github.com/davidea97/Multi-Camera-Hand-Eye-Calibration.git.

==> tex/3_method_old.tex <==
%In this paper, we tackle the challenge of multi-camera hand-eye calibration in industrial robotic workcells, formulating a non-linear optimization algorithm based on re-projection error minimization. This aims to estimate the rototranslation between each sensor and the manipulator base in a single optimization procedure, leveraging on additional constraints in the optimization, specifically the unique board-to-hand transformation shared by all cameras and the spatial constrains between cameras. 
%
% --- MT riscritto sotto
%This section introduces our novel multi-camera hand-eye calibration method that generalizes the single-camera hand-eye calibration technique described in~\cite{evangelista2022unified} to configurations involving multiple cameras. The proposed hand-eye calibration of multi-camera systems is based on minimizing the re-projection error and it incorporates two critical elements into the optimization: (i) a single transformation between the calibration pattern and the robot's end-effector removing the need for calculating that transformation independently for each camera and (ii) the spatial transformation among the cameras ensuring consistency among all relative transformations between the cameras and the robot base.
This section introduces our novel multi-camera hand-eye calibration method, that generalizes the approach introduced in~\cite{evangelista2022unified} to configurations involving multiple cameras. As in~\cite{evangelista2022unified}, our calibration method is based on the minimization of the re-projection error by means of non-linear optimization, but it introduces two main constraints into the optimization: (i) a single transformation between the calibration pattern and the robot's end-effector removing the need for calculating that transformation independently for each camera and (ii) the spatial transformation among the cameras ensuring consistency among all relative transformations between the cameras and the robot base.
%
Section \ref{subsec:single_calib} briefly summarizes the single-camera hand-eye calibration work proposed in \cite{evangelista2022unified}, presenting the main notations that will be adopted for the formulation of our method. In Section \ref{subsec:multi_calib}, a comprehensive and detailed explanation of the proposed multi-camera hand-eye calibration method is described.
The hand-eye calibration methods discussed in the following sections make use of the Ceres Solver library, well-suited to solve large and complex non-linear optimization problems.


%%%%%%%%%%% SUBSECTION: Single-camera calibration %%%%%%%%%%

\subsection{Single-camera hand-eye calibration}
\label{subsec:single_calib}
In \cite{evangelista2022unified} we presented an hand-eye calibration technique which does not rely on the PnP algorithm but rather solves the calibration through the minimization of the re-projection error. Its main purpose is to estimate the unknown rototranslations $X$ and $Z$, illustrated in Fig. \ref{fig:single_camera_setup}. This method aims to minimize the objective function $c$ reported in (\ref{eq:cost_function}).
%
\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{ieeeconf/images/single_camera1.pdf}
  \caption{Transformations chain in a single-camera hand-eye setup, illustrating the re-projection of calibration pattern corners onto the image plane. The robot's end effector pose relative to its base (W) is denoted by $T_{E}^{W}$, along with two unknown matrices: $X$, representing the hand-eye transformation, and $Z$, denoting the transformation between the board and the robot's end-effector pose.}
  \label{fig:single_camera_setup}
\end{figure}
%
The cost function $c$ represents the euclidean distance between the detected 2D corners \mbox{$p_{ij}^{D}=(u_{x}, u_{y})_{ij}^{D}$} of the calibration pattern and their corresponding 3D corners re-projected on the image plane, denoted by $(u_{x}, u_{y})_{ij}^{P}$.
\begin{equation}
     c = \sum_{j=0}^{M-1}\sum_{i=0}^{L-1} \left\|{\begin{pmatrix} u_{x} \\ u_{y} \end{pmatrix}_{ij}^{\mathrm{P}}-\begin{pmatrix} u_{x} \\ u_{y} \end{pmatrix}_{ij}^{\mathrm{D}}}\right\|^{2}
    \label{eq:cost_function}
\end{equation}
Here, $j=0,\dots,M-1$ denotes the $j^{th}$ pose of the robot's end-effector with respect to its base and $i=0,\dots,L-1$ is the $i^{th}$ corner of the calibration pattern.
Hence, consider the 3D control points of a calibration target, denoted as $P_{i}^{B}=(X_{i},Y_{i},Z_{i})$, along with the function $f_{k}$ that models the camera's projection, such as the pinhole camera model, for a given camera $C_k$ in the calibration process. In this process, two key transformations are calculated at each optimization step: the hand-eye transformation $T_{W}^{C_{k}}$, and the rototranslation $[T_{B}^{E}]_{k}$ from the calibration board to the robot's end-effector for camera $C_k$.
%the hand-eye transformation $T_{W}^{C_{k}}$ and the rototranslation board-to-hand $[T_{B}^{E}]_{k}$ are the two unknown transformations that are estimated in each optimization step: 
The single-camera hand-eye calibration method aims to minimize the difference between the projected control points and their detected positions in the camera's image plane, as outlined in the equation in~(\ref{eq:minimization_eq}). 
\begin{equation}
    %\underset{T_{W}^{C},T_{B}^{E}}{\mathrm{argmin}} 
    c_{k} = \sum_{j=0}^{M-1}\sum_{i=0}^{L-1}\left\|{f_{k}(T_{W}^{C_{k}} [T_{E}^{W}]_{j} [T_{B}^{E}]_{k}) P_{i}^{B}-p_{ijk}^{D}}\right\|^{2}
    \label{eq:minimization_eq}
\end{equation}
Here, the geometric transformation $[T_{E}^{W}]_{j}$ denotes the $j^{th}$ pose of the end-effector with respect to the robot base, achieved by the robot arm during the image acquisition, provided by its direct kinematics. 

%In the context of a camera network covering a robot workcell, cameras are typically strategically positioned to minimize occlusions and maximize overlapping fields of view (FoV). In such scenarios, multiple cameras often capture images of the same calibration pattern simultaneously.

%However, running the single-camera hand-eye calibration independently for each sensor prove not to be robust at all, as discussed in Section~\ref{sec:experiments}. This is because, in each optimization process, a new board-to-hand transformation $[T_{E}^{B}]_{k}$ is estimated ignoring the fact that it is fixed and shared by each sensor. Additionally, the recovery of camera-to-camera transformations relies on individual hand-eye transformations $T_{W}^{C_{k}}$, leading to error propagation. This approach introduces higher inaccuracies since it exclusively relies on a single-camera image collection process at a time. If, by chance, the collected data is affected by noise, possibly due to inaccurate pattern detection, it can result in an erroneous calibration of the sensor. In contrast, in a camera network setup within a robotic workcell, cameras are strategically positioned to minimize occlusions and maximize field of view (FoV) overlap. Additionally, they often capture images of the same calibration pattern simultaneously, offering the opportunity to leverage information from multiple cameras concurrently for a more robust calibration process.

%However, running an algorithm that performs single-camera calibration $N$ times, where $N$ is the number of sensors in a camera network, proves to be suboptimal solution as it is analyzed in Section~\ref{sec:experiments}. This is because, in each optimization process, a new board-to-hand transformation $[T_{E}^{B}]_{k}$ is estimated ignoring the fact that it is fixed and shared by each sensor. Moreover camera-to-camera is recovered using the individual hand-eye transformations $T_{W}^{C_{k}}$, leading to the error propagation. However, when considering a camera network covering a robot workcell, usually cameras are positioned in order to reduce occlusions and to maximize overlapping of their field of view (FoV). In such scenario, when images of the known pattern are taken by all the cameras, it is quite common that more cameras frame the same pattern; this means that the simultaneous detection of the calibration pattern by different cameras is not taken into account, increasing the inaccuracy of this approach, because of relying on a collection of images of a calibration pattern captured by a single camera which can be affected by some noise reducing the accuracy of corner detections and consequently affecting the final calibration. 

\subsection{Multi-camera hand-eye calibration}
\label{subsec:multi_calib}

%In this paper, we generalized the single-camera hand-eye calibration for dealing with multi-camera setups, enabling the calibration of an entire camera network in relation to the robot manipulator. While single-camera hand-eye calibration, aims to calibrate independently each camera using its own images, the proposed method leverages all images from all cameras simultaneously during the optimization process. 
Building upon the formulation described in Sec.~\ref{subsec:single_calib} for the calibration of a single-camera, our method tackles the problem of calibrating multi-camera systems with respect to the robot, leveraging the availability of all images gathered from all cameras simultaneously during the optimization step.
\begin{figure}
  \centering
  \includegraphics[width=0.99\linewidth]{ieeeconf/images/multi_camera1.pdf}
  \caption{Multi-camera hand-eye setup, illustrating the geometric transformations optimized through the proposed multi-camera hand-eye calibration method. They include the single board-to-hand transformation common to all cameras, the spatial constraints among the cameras, and all the hand-eye transformations.}
  \label{fig:multi_camera_setup}
\end{figure}
%In particular, when the checkerboard is detected concurrently by multiple cameras, as illustrated in Fig.~\ref{fig:multi_camera_setup}, this collective information plays a key role to introduce two additional constraints in the optimization procedure: the unified pattern-to-hand transformation $T_{B}^{E}$ that is shared by all cameras and the spatial constraint $T_{C_{t}}^{C_{k}}$ that exists between cameras.
When the checkerboard is concurrently detected by multiple cameras, as depicted in Fig.~\ref{fig:multi_camera_setup}, the collective images taken by all cameras become crucial. This scenario allows to introduce the two aforementioned additional constraints in the optimization procedure: the single board-to-hand transformation $T_{B}^{E}$ and the spatial constraint $T_{C_{t}}^{C_{k}}$ that defines the geometric transformation between cameras $k$ and $t$.
%The proposed multi-camera hand-eye calibration algorithm involves a single non-linear optimization process for calibrating an entire camera network with respect to the robot manipulator. 
%In particular, the proposed multi-camera hand-eye calibration is innovative because it aims to minimize two main objective functions: not only the $c_{rpj}$ function centred on the reprojection error of each individual camera, but it also aims to minimise $c_{cross}$, which optimizes the spatial transformations existing between cameras as defined in~(\ref{eq:final_optimization}). 
The proposed multi-camera hand-eye calibration approach stands out for its innovative strategy that seeks to minimize two principal objective functions simultaneously. The first function, denoted as $c_{rpj}$, represents the re-projection error for each individual camera, and its minimization ensures the precise alignment between the observed and the re-projected control points within each camera's image plane. The second objective, $c_{cross}$, is dedicated to optimizing the spatial transformations between the cameras, enhancing the consistency and accuracy of their relative positions and orientations. The final objective function is outlined in~(\ref{eq:final_optimization}).
\begin{equation}
    \underset{T_{C_{t}}^{C_{k}}, T_{W}^{C_{t}},T_{B}^{E}}{\mathrm{argmin}} \, c_{cross} + c_{rpj}
    \label{eq:final_optimization}
\end{equation}
%represents the re-projection error for each camera detecting the calibration pattern at the $j^{th}$ robot pose, ,. This
The cost function $c_{rpj}$ leverages the shared board-to-hand transformation $T_{B}^{E}$, common across all cameras, as detailed in (\ref{eq:c1}). This function is incorporated into the optimization process, taking into account every camera that records the calibration pattern at the robot's $j^{th}$ pose. 
\begin{equation}
    c_{rpj} = \sum_{j=0}^{M-1}\sum_{k=0}^{N-1}\sum_{i=0}^{L-1} \left\| f_{k}(T_{W}^{C_{k}}[T_{E}^{W}]_{j}T_{B}^{E}) P_{i}^{B} - p_{ijk}^{D} \right\|^{2}
    \label{eq:c1}
\end{equation}
%On the other hand, the objective function $c_{cross}$ defined in (\ref{eq:c2}), focuses on minimizing the re-projection error aiming to optimize the relative transformations among cameras. This is crucial when cross-detections occur, that is, when the checkerboard is simultaneously detected by multiple cameras.
On the other hand, the objective function $c_{cross}$, as specified in (\ref{eq:c2}), aims to minimize the difference between control points detected by camera $k$ and their re-projection onto this camera's image plane through camera $t$. This process is key for refining the relative transformations $T_{C_{t}}^{C_{k}}$ between the cameras, exploiting the occurrence of cross-detections, i.e. when the checkerboard is simultaneously detected by more cameras.
\begin{equation}
    c_{cross} = \sum_{j=0}^{M-1}\sum_{k=0}^{N-1}\sum_{t=0}^{N-1}\sum_{i=0}^{L-1} \left\| p_{ijk}^{cross} - p_{ijk}^{D} \right\|_{2}
    \label{eq:c2}
\end{equation}

A cross-detection matrix $\mathbf{X}_j$ is used within the optimization framework to describe when two cameras are jointly detecting the calibration pattern . This matrix consists of binary values in each cell, $\mathbf{X}_j(k, t)$, where $k\neq t$, indicating the concurrent detection of the calibration pattern by cameras $k$ and $t$ at the $j^{th}$ time step. Consequently, the re-projected corners $p_{ijk}^{cross}$ can be computed as shown in (\ref{eq:cross_proj}).
%where the transformation $T_{C_{t}}^{C_{k}}$ from camera $t$ to camera $k$ is incorporated.
\begin{equation}
    p_{ijk}^{cross} = f_{k}(T_{C_{t}}^{C_{k}}T_{W}^{C_{t}}[T_{E}^{W}]_{j}T_{B}^{E})P_{i}^{B} \cdot\mathbf{X}_{j}(k,t)
    \label{eq:cross_proj}
\end{equation}
%Therefore, the final multi-camera hand-eye calibration method can be mathematically formalized as defined in (\ref{eq:final_optimization}).
%\begin{equation}
%    \underset{T_{C_{t}}^{C_{k}}, T_{W}^{C_{t}},T_{B}^{E}}{\mathrm{argmin}} \, c_{cross} + c_{rpj}
%    \label{eq:final_optimization}
%\end{equation}
%The iterative Schur solver was used to solve the optimization problem driven by the Cauchy loss function which is less sensitive to outliers. Moreover the Levenberg-Marquardt algorithm was adopted which has the main advantage of introducing a regularization parameter to control the step size during the optimization process. This parameter ensures stability and convergence of the algorithm, particularly in cases where the Gauss-Newton method might encounter issues, such as when the curvature of the objective function is ill-conditioned.

To our knowledge, this is the first multi-camera hand-eye calibration that takes advantage of both constraints through a non-linear optimization algorithm. Moreover, the optimization problem, is guided by the robust Cauchy loss function to enhance resilience against outliers.
%The optimization problem, guided by the robust Cauchy loss function to enhance resilience against outliers, was addressed using the Levenberg-Marquardt algorithm \cite{more2006levenberg} for its property of incorporating a regularization parameter to govern the step size in the optimization process. This parameter plays a crucial role in ensuring the stability and convergence of the algorithm~\cite{gavin2019levenberg}.


%Notably, our method outperforms other state-of-the-art multi-camera hand-eye calibration methods and also single-camera hand-eye calibration algorithms applied individually to each camera, especially in challenging real-world scenarios such as industrial robotic workcells. Furthermore, our approach demonstrates superior speed, outperforming existing multi-camera calibration methods in terms of both the execution time of the optimization process and the number of images required for calibration. This speed advantage is particularly significant, as many existing methods in the literature struggle with prolonged calibration times and a high demand for calibration pattern images to achieve acceptable accuracy.

%In the Sec.~\ref{sec:experimental}-\ref{sec:robustness} it can be observed that this method allows to calibrate a multi-camera setup with respect to the robot through a single process significantly improving the calibration performance and outperforming the single-camera calibration from the robustness point of view with fewer limits on the initial guess with respect to the other methods of Sec.~\ref{subsec:single_calib}, ~\ref{subsec:multi_calib_woc} and other methods of the state of the art.
%si parte da metodo ETFA, e si estende introducedno due ipotesi: trasformata hand-eye in comune + vincoli tra telecamere
